Security Issues of Low Power Wide Area Networks in the Context of LoRa Networks

Low Power Wide Area Networks (LPWAN) have been used to support low cost and mobile bi-directional communications for the Internet of Things (IoT), smart city and a wide range of industrial applications. A primary security concern of LPWAN technology is the attacks that block legitimate communication between nodes resulting in scenarios like loss of packets, delayed packet arrival, and skewed packet reaching the reporting gateway. LoRa (Long Range) is a promising wireless radio access technology that supports long-range communication at low data rates and low power consumption. LoRa is considered as one of the ideal candidates for building LPWANs. We use LoRa as a reference technology to review the IoT security threats on the air and the applicability of different countermeasures that have been adopted so far. LoRa nodes that are close to the gateway use a small SF than the nodes which are far away. But it also implies long in-the-air transmission time, which makes the transmitted packets vulnerable to different kinds of malicious attacks, especially in the physical and the link layer. Therefore, it is not possible to enforce a fixed set of rules for all LoRa nodes since they have different levels of vulnerabilities. Our survey reveals that there is an urgent need for secure and uninterrupted communication between an end-device and the gateway, especially when the threat models are unknown in advance. We explore the traditional countermeasures and find that most of them are ineffective now, such as frequency hopping and spread spectrum methods. In order to adapt to new threats, the emerging countermeasures using game-theoretic approaches and reinforcement machine learning methods can effectively identify threats and dynamically choose the corresponding actions to resist threats, thereby making secured and reliable communications.

==> Attack_LoRa.tex <==
\section{Security threats of LoRa Network}
There are several survey papers~\cite{makhdoom2018anatomy, tomic2017survey, GuWWirelessSurvey2011, ChahidIoTProtocol2017} that have discussed the security threats in the wireless network. They have broadly divided the network into WLAN (using WiFi technologies)~\cite{afanasyev2010usage}, WSN (using Zigbee and Bluetooth)~\cite{suryadevara2012wireless, mackensen2012bluetooth} and Ad-hoc wireless networks~\cite{sarkar2016ad}. Normally these kinds of networks have a short range (100 meters). WiFi has a high data rate (100 Mbps) while WSN Zigbee has low data rates (250 kbps). LoRa is meant to cover at least 1-2 miles and therefore has a very low data rate (50 kbps) but long on-air time. It makes LoRa susceptible to different DoS and MITM attacks.

% Each of these network types has unique properties and therefore different security risks. 


% The long transmission time caused by the low data rate makes the LoRa wireless links venerable to jamming attacks. 
%  LoRa end-devices that use the lowest data rate at the edge of communication range are susceptible to these kind of attacks. Current research work suggests \cite{aras2017selective} that off-the-shelf LoRa commodity hardware can be used to perform these attacks. In addition, LoRa message headers are not encrypted which allow an attacker to identify the source sensor device, class of traffic, etc.
%  Among the three types of jamming attacks, triggered or continuous jamming is the most common form of attack that affects all messages in a frequency band. Therefore it can be easily thwart by the network administrator and the affected bands can be marked as jammed. 
% Selective jamming can listen on the channels, target a particular device or traffic class and then jam selected messages.The jamming policy is only concerned with content following the physical header. Selective jamming can prevent critical messages from reaching the gateway, especially for those sensor devices that only transmit when the sensor state change happens (event driven sensors).
% \textit{Wormhole attack with selective jamming} can elevate the threat level by adding message replay capability. There is no time-related information in LoRaWAN message header and only loose timing requirement due to LoRa\textsc{}'s long transmission time.  Therefore, messages can be recorded, jammed and then can be replayed later to appear as a valid message as long as a message with a higher sequence number is received at the gateway. It is a severe security threat to critical application in the health-care, industrial, and power systems industries. All these issues are discussed in the following subsections

\subsection{DoS attack by jamming LoRa networks}
Recently, there are a few papers on the security analysis of LoRa networks~\cite{aras2017selective,naoui2016enhancing,tomasin2017security}; however, the large portion of security challenges are not yet addressed.  In \cite{altolini2013low}, the authors present a comprehensive study on the link-layer security functions of low power IoT networks and find that having the AES ciphers implemented in the hardware chips reduces the memory and power demand. In the physical layer, LoRa is susceptible to jamming attacks which can be carried out by low-cost commodity hardware broadcasting LoRa messages \cite{aras2017selective}. Jamming is a widely studied research issue of wireless networks such as WiFi, Zigbee, and Bluetooth. The three broad categories of jamming attacks are triggered jamming, selective jamming, and wormhole attack.
% \\LPWAN poses unique security challenges due to its network model and security compromises for low power requirement. 

% LoRa suffers from the coexistence problem as LoRa does not employ channel sensing and the transmission of LoRa messages is long. 

\subsubsection{Triggered and continuous jamming}
The jamming attack is a widely used and potent attack to disrupt a regular radio communication by deliberately causing interference in the channel and reducing the overall signal to noise ratio (SNR) at the receiver. It can increase the packet collision rate by injecting malicious packets in the network, causing nodes to re-transmit and quickly exhaust battery power. Overall, legitimate nodes will be barred from sending messages. There are broadly three classes of jamming attacks that have been used to attack many networks \cite{aras2017exploring}.

This kind of attack affects all devices on a specific frequency. The attacking device only needs to detect the preamble of a LoRa MAC packet and triggers the jamming mechanism so that the packet never reaches the intended gateway. This attack can be identified easily by the network administrator due to high packet drop rate on a particular frequency and can be marked as jammed.
\subsubsection{Selective jamming}
Selective jamming not only reads through the preamble but also the message header. Thus attackers can listen on the channels, target a particular device or traffic class and then jam selected messages~\cite{aras2017exploring,proano2010selective}.
In order to selectively jam LoRaWAN messages, an attacker has to perform the following steps. It first detects a LoRaWAN packet. It aborts receiving if the received content triggers the jamming policy (usually first 5 bytes).
If no, it immediately jams the channel.  Therefore, the jamming window is smaller than the regular triggered jamming.
However, selective jamming can prevent critical messages from reaching the gateway, especially for those sensor devices that only transmit when the sensor state change happens (event-driven sensors). Selective jamming is implemented on a real test-bed with cheap hardware \cite{aras2017selective}.
 \subsubsection{Selective jamming with Wormhole attack}
 Classical wormhole attack requires two malicious devices in a wireless sensor network \cite{YHuWormhole2003,MpriyaWormhole2012}. One device records regular network messages and tunnels them to the other device through a low-latency network.  Generally, this kind of attack is meant for mesh networks where false routing information is created to drain out the energy of the network. The classical wormhole attack is not suitable for LoRaWAN that uses the star topology. However, there is no time-related information in LoRaWAN message header and only loose timing requirement due to LoRa'’s long transmission time.
Therefore, messages can be recorded, jammed, and then can be replayed later to appear as a valid message as long as a message with a higher sequence number is received at the gateway.
In this kind of selective jamming and wormhole attack, two devices are involved and act as a sniffer and a jammer separately. The sniffer receives the messages and decides whether to jam as per normal jamming policy. If the decision to jam is made, it signals to the jammer using a low latency network to jam the message immediately. The sniffer constantly sniffs the network. In order to carry out this kind of attack, the following steps are followed by the sniffer and the jammer.

The sniffer first detects a LoRaWAN packet
and starts receiving and recording the packet. By receiving a packet, it sends a signal through a low latency (better than LoRaWAN) to the jammer. By receiving the signal from the sniffer, the jammer turns to the active mode.

By replaying the recorded regular messages while jamming, the attacker not only intercepts the state change alert messages but also makes it look like nothing out of the ordinary has happened. The window of opportunity in this kind of attack is even lower than selective jamming as there are two devices involved. Devices that are using high SF and therefore, long on-air transmission time are more vulnerable to this kind of attack.

\begin{figure}[t]
\begin{center}
	\includegraphics[scale= 0.50]{Figures/LoRaOnAirTime_2.png}
\end{center}
   	\caption{\textbf{Time available to jam for various packet sizes for each SF}}
	\label{fig:LoRaOnAirTime_2}
	 \vspace{-15pt}
\end{figure}

Small scale experiments with wormhole attacks have been carried out in recent times as literature suggests \cite{aras2017selective}. The most critical aspect of a successful attack is that the reaction time of the jammer must be less than the on-air time of the LoRaWAN packet reduced by the message header bytes. In \cite{aras2017selective}, the mean reaction time of jammer is experimentally found to be 100 milliseconds. 
Fig. \ref{fig:LoRaOnAirTime_2} shows the time available to jam for various packet sizes for different SF when the mean reaction time is 100 milliseconds. It can be observed that LoRa devices that are on the edge of the network and using higher SF are more vulnerable to such kinds of jamming attacks.
This section shows that the threats to all LoRa devices are not the same as they are not equally vulnerable. End devices that are using low data rate or high SF have longer on-air time and prone to these kinds of jamming attacks. Jamming causes packet drop, the transmission of lost packets and overall higher energy consumption of sensor nodes. End devices adjust their data rate based on the distance from the gateway. There is no intelligence, neither in the gateway or in the end devices which might sit on top of the adaptive data rate that can adjust the transmission parameters to counter the attack.

Packet drop can also happen due to the collision of packets due to the standard ALOHA protocol. There is no mechanism or method in place to distinguish between losses due to malicious attacks and collisions.





